A Programmatic and Semantic Approach to Explaining and DebuggingNeural Network Based Object Detectors

Even as deep neural networks have become very effective for tasks in vision and perception, it remains difficult to explain and debug their behavior. In this paper, we present a programmatic and semantic approach to explaining, understanding, and debugging the correct and incorrect behaviors of a neural network-based perception system. Our approach is semantic in that it employs a high-level representation of the distribution of environment scenarios that the detector is intended to work on. It is programmatic in that scenario representation is a program in a domain-specific probabilistic programming language which can be used to generate synthetic data to test a given perception module. Our framework assesses the performance of a perception module to identify correct and incorrect detections, extracts rules from those results that semantically characterizes the correct and incorrect scenarios, and then specializes the probabilistic program with those rules in order to more precisely characterize the scenarios in which the perception module operates correctly or not. We demonstrate our results using the SCENIC probabilistic programming language and a neural network-based object detector. Our experiments show that it is possible to automatically generate compact rules that significantly increase the correct detection rate (or conversely the incorrect detection rate) of the network and can thus help with understanding and debugging its behavior.

==> sections/limitations.tex <==
% \documentclass[../main.tex]{subfiles}

The expressiveness and interpretability of \scenic language is enhanced by leveraging detailed information about the map used in the simulator. For example, in Scenario 1 as shown in Figure \ref{fig:supp_scenario1_2}(a), we can directly refer to specific part of the road such as ''curb'' because we have already identified the curb regions in the map. And, description on placing of ''otherCar'' with respect to a spot on curb makes the program easily understandable to human. However, because GTA-V is not an open sourced simulator (in fact it is not even meant to be used as a simulator but is widely used for its realistic rendering), we could not parse out detailed map information such as regions of different lanes, location of traffic lights, etc. As the number of cars scaled, describing increasingly complicated geometric relations among cars without any reference points/objects/regions, such as lanes, became more challenging. As a result, we were limited to describe geometric relations in scenarios by only referencing cars, which resulted in much less understandable \scenic programs, deprecating the use of \scenic as a scenario description. We emphasize that this limitation due to inaccessible map information of the simulator, not \scenic. In fact, \scenic has syntax to refer to other entities in the scene if those information are accessible in the simulator's map. Such reference would significantly enhance the interpretability of the \scenic programs we generate with our method.
